How to Upscale Neural Networks with Scaling Law? A Survey and Practical Guidelines

Neural scaling laws have revolutionized the design and optimization of large-scale AI models by revealing predictable relationships between model size, dataset volume, and computational resources. Early research established power-law relationships in model performance, leading to compute-optimal scaling strategies. However, recent studies highlighted their limitations across architectures, modalities, and deployment contexts. Sparse models, mixture-of-experts, retrieval-augmented learning, and multimodal models often deviate from traditional scaling patterns. Moreover, scaling behaviors vary across domains such as vision, reinforcement learning, and fine-tuning, underscoring the need for more nuanced approaches. In this survey, we synthesize insights from over 50 studies, examining the theoretical foundations, empirical findings, and practical implications of scaling laws. We also explore key challenges, including data efficiency, inference scaling, and architecture-specific constraints, advocating for adaptive scaling strategies tailored to real-world applications. We suggest that while scaling laws provide a useful guide, they do not always generalize across all architectures and training strategies.

==> tables/practical_guidelines.tex <==
\begin{table*}[h]
   \centering
   \begin{tabular}{|p{4cm}|p{6cm}|p{4cm}|}
       \cline{1-3}
       \textbf{Scaling Aspect} & \textbf{Guideline} & \textbf{Key Reference} \\
       \cline{1-3}
       \textbf{Model-Data Scaling} & Balance model parameters and data size using Chinchilla scaling laws; prioritize data scaling for compute-limited scenarios. & \citep{hoffmann_training_2022} \\
       \cline{1-3}
       \textbf{Compute Efficiency} & Optimize training compute via retrieval-based architectures, MoEs, and adaptive test-time compute strategies. & \citep{brown_large_2024} \\
       \cline{1-3}
       \textbf{Training Duration} & Longer training with repeated data exposure (4-16 epochs) is more effective than parameter expansion. & \citep{muennighoff_scaling_2023} \\
       \cline{1-3}
       \textbf{Sparse vs. Dense Models} & Sparse Mixture of Experts (MoE) models can achieve up to 40× compute efficiency gains compared to dense models. & \citep{krajewski_scaling_2024} \\
       \cline{1-3}
       \textbf{Data Composition} & Use REGMIX and AUTOSCALE to optimize data mixtures dynamically based on model scale. & \citep{liu_regmix:_2024, kang_autoscale:_2024} \\
       \cline{1-3}
       \textbf{Inference Optimization} & Use tree search and retrieval augmentation to allow smaller models to match larger models’ performance. & \citep{wu_inference_2024} \\
       \cline{1-3}
       \textbf{Quantization} & 4-bit precision optimizes zero-shot performance while reducing compute costs. & \citep{dettmers_case_2023} \\
       \cline{1-3}
   \end{tabular}
   \label{tab:scaling_guidelines}
      \caption{Scaling Strategies and Practical Recommendations}
\end{table*}

==> tables/reproducibility.tex <==
% Table generated by Excel2LaTeX from sheet 'Reproducibility_avail'
\begin{table*}[htbp]
  \centering
  \scalebox{0.7}{
    \begin{tabular}{l c c c c c}
    \cline{1-6}
    \textbf{Paper} & \textbf{Training Code?} & \textbf{Analysis Code?} & \textbf{Checkpoints?} & \textbf{Metric Scores?} & \multicolumn{1}{l}{\textbf{Github}} \\
    \cline{1-6}
    \citet{mikami_scaling_2021} & N     & Y     & Y     & Y     & \multicolumn{1}{l}{\href{https://github.com/pfnet-research/cg-transfer}{Link}} \\
    \citet{sardana_beyond_2024} & N     & N     & N     & N     &  \\
    \citet{sorscher_beyond_2023} & N     & N     & N     & Y     &  \\
    \citet{caballero_broken_2023} & N     & Y     & N     & Y     & \multicolumn{1}{l}{\href{https://github.com/ethancaballero/broken_neural_scaling_laws}{Link}} \\
    \citet{hu_minicpm:_2024} & Y     & N     & N     & N     & \multicolumn{1}{l}{\href{https://github.com/OpenBMB/MiniCPM/tree/main}{Link}} \\
    \citet{alabdulmohsin_revisiting_2022} & N     & N     & Y     & N     & \multicolumn{1}{l}{\href{https://github.com/google-research/google-research/tree/master/revisiting_neural_scaling_laws}{Link}} \\
    \citet{gao_scaling_2024} & Y     & Y     & Y     & N     & \multicolumn{1}{l}{\href{https://github.com/EleutherAI/sparsify}{Link}} \\
    \citet{muennighoff_scaling_2023} & Y     & N     & N     & N     & \multicolumn{1}{l}{\href{https://github.com/huggingface/datablations}{Link}} \\
    \citet{hernandez_scaling_2021} & N     & N     & N     & N     &  \\
    \citet{neumann_scaling_2023} & Y     & Y     & Y     & N     & \multicolumn{1}{l}{\href{https://github.com/OrenNeumann/AlphaZero-scaling-laws}{Link}} \\
    \citet{henighan_scaling_2020} & N     & N     & N     & N     &  \\
    \citet{aghajanyan_scaling_2023} & N     & N     & N     & N     &  \\
    \citet{kaplan_scaling_2020} & N     & N     & N     & N     &  \\
    \citet{hilton_scaling_2023} & N     & N     & N     & N     &  \\
    \citet{frantar_scaling_2023} & N     & N     & N     & N     &  \\
    \citet{tay_scaling_2022} & N     & N     & N     & N     &  \\
    \citet{zhai_scaling_2022} & Y     & N     & N     & N     & \multicolumn{1}{l}{\href{https://github.com/google-research/big_vision}{Link}} \\
    \citet{hoffmann_training_2022} & N     & N     & N     & N     &  \\
    \citet{clark_unified_2022} & N     & N     & N     & N     &  \\
    \cline{1-6}
    \end{tabular}%
    }
  \label{tab:reproducibility}%
  \caption{Reproducibility of different neural scaling law papers.}
\end{table*}%

